5G Multimedia Massive MIMO Communications Systems

In the Fifth generation (5G) wireless communication systems, a majority of the traffic demands is contributed by various multimedia applications. To support the future 5G multimedia communication systems, the massive multiple-input multiple-output (MIMO) technique is recognized as a key enabler due to its high spectral efficiency. The massive antennas and radio frequency (RF) chains not only improve the implementation cost of 5G wireless communication systems but also result in an intense mutual coupling effect among antennas because of the limited space for deploying antennas. To reduce the cost, an optimal equivalent precoding matrix with the minimum number of RF chains is proposed for 5G multimedia massive MIMO communication systems considering the mutual coupling effect. Moreover, an upper bound of the effective capacity is derived for 5G multimedia massive MIMO communication systems. Two antenna receive diversity gain models are built and analyzed. The impacts of the antenna spacing, the number of antennas, the quality of service (QoS) statistical exponent, and the number of independent incident directions on the effective capacity of 5G multimedia massive MIMO communication systems are analyzed. Comparing with the conventional zero-forcing precoding matrix, simulation results demonstrate that the proposed optimal equivalent precoding matrix can achieve a higher achievable rate for 5G multimedia massive MIMO communication systems.

==> WCMAUTH.tex <==
%---------------------------------------------------------------------------
%Please  be  aware that the use of this LaTeX class file is governed by the
%following conditions:
%
% based on the original LaTeX ARTICLE DOCUMENT STYLE
% Copyright (C) 1988, 1989 by Leslie Lamport
%
% Copyright (c) 2010 John Wiley & Sons, Ltd, The Atrium, Southern Gate, Chichester,
% West Sussex, PO19 8SQ UK.   All rights reserved.
%
%Rules of Use
%
%% You are NOT ALLOWED to change this file.
%
%
%This class file is made available for use by authors who wish to prepare an
%article for publication in
%WIRELESS COMMUNICATIONS AND MOBILE COMPUTING
%published by John Wiley & Sons Ltd. The user may not exploit any part of
%the class file commercially.
%
%This class file is provided on an `as is'  basis, without warranties of any
%kind, either expressed or implied, including but not limited to warranties of
%title, or  implied warranties of merchantablility or fitness for  a
%particular purpose. There will be no duty on the author[s] of the software
%or John Wiley & Sons Ltd to correct any errors or defects in the software.
%Any statutory rights you may have remain unaffected by your acceptance of
%these rules of use.
%---------------------------------------------------------------------------
%
% Created by Alistair Smith, Sunrise Setting Ltd, 01 July 2010
%
% wcmauth.cls --- For Wirel. Commun. Mob. Comput.

\def\update{2010/07/01 v2.00}

\newcommand{\journalname}{WIRELESS COMMUNICATIONS AND MOBILE COMPUTING}
\newcommand{\journalnamelc}{Wireless Communications and Mobile Computing}
\newcommand{\journalabb}{Wirel. Commun. Mob. Comput.}
\newcommand{\journalclass}{wcmauth.cls}
\newcommand{\journalclassshort}{wcmauth}
\newcommand{\DOI}{wcm}

\NeedsTeXFormat{LaTeX2e}
\ProvidesClass{wcmauth}[\update\ \journalclass]

%\newcommand\hmmax{0}

\newif\if@timesfont
\DeclareOption{times}{%
\@timesfonttrue}

\newif\if@doublespace
\DeclareOption{doublespace}{%
\@doublespacetrue}

\DeclareOption*{\PassOptionsToClass{\CurrentOption}{article}}
\ProcessOptions
\LoadClass{article}
\if@timesfont
\RequirePackage{times}
\fi
\if@doublespace
\RequirePackage[onehalfspacing]{setspace}
\fi

\RequirePackage{graphicx}
\RequirePackage{pifont,latexsym,ifthen,rotating,calc,textcase,booktabs,color}
\RequirePackage{amsfonts,amssymb,amsbsy,amsmath,amsthm}
%\RequirePackage{bm}
\RequirePackage[errorshow]{tracefnt}

\@twosidetrue
\flushbottom
\frenchspacing

\textwidth 36.5pc
\textheight 636pt
\setlength\columnsep{18pt}

%Trim sizes
\setlength\voffset{-1in}
\setlength\hoffset{-1in}
\topmargin -1mm
\setlength\oddsidemargin{33mm}%back margin on odd pages
\setlength\evensidemargin{33mm}%fore margin on even pages
\setlength\paperwidth{210mm}
\setlength\paperheight{276mm}
%Needed to set PDF page size
\special{papersize=210mm,276mm}

\parskip \z@
\parindent 1em
\headheight 50pt
\headsep    20pt
\footskip 28pt

\hyphenpenalty=1000
\pretolerance=8000
\tolerance=9500
\hbadness=8000
\vbadness=9000
\displaywidowpenalty=0
\clubpenalty=10000
\widowpenalty=10000
\lefthyphenmin=3%
\righthyphenmin=3%
\brokenpenalty=10000%

\thinmuskip = 3mu
\medmuskip = 4mu
\thickmuskip = 5mu

\setcounter{topnumber}{10}
\def\topfraction{1}
\setcounter{bottomnumber}{10}
\def\bottomfraction{0.8}
\setcounter{totalnumber}{10}
\def\textfraction{0}
\renewcommand{\floatpagefraction}{0.95}
\setcounter{dbltopnumber}{10}
\renewcommand{\dblfloatpagefraction}{0.95}
\renewcommand{\dbltopfraction}{1}

\renewcommand\normalsize{%
   \@setfontsize\normalsize\@ixpt{11pt}%
   \abovedisplayskip 10\p@ \@plus2\p@ \@minus5\p@
   \abovedisplayshortskip \z@ \@plus3\p@
   \belowdisplayshortskip 6\p@ \@plus3\p@ \@minus3\p@
   \def\@listi{\leftmargin\leftmargini
               \topsep 6\p@ \@plus2\p@ \@minus2\p@
               \parsep 3\p@ \@plus2\p@ \@minus\p@
               \itemsep \parsep}%
   \belowdisplayskip \abovedisplayskip
}
\normalsize

\renewcommand{\small}{\fontsize{7.5pt}{9.5pt}\selectfont}
\renewcommand{\footnotesize}{\fontsize{6.5pt}{8.5pt}\selectfont}
\renewcommand\scriptsize{\@setfontsize\scriptsize\@viipt{9.5}}
\renewcommand\tiny{\@setfontsize\tiny\@vpt\@viipt}
\renewcommand\large{\@setfontsize\large\@xipt{13}}
\renewcommand\Large{\@setfontsize\Large\@xivpt{18}}
\renewcommand\LARGE{\@setfontsize\LARGE\@xviipt{22}}
\renewcommand\huge{\fontsize{22pt}{24pt}\selectfont}
\renewcommand\Huge{\@setfontsize\Huge\@xxvpt{30}}

\newcommand{\numsize}{\fontsize{8pt}{10pt}\selectfont}
\newcommand{\titlesize}{\fontsize{15pt}{18pt}\selectfont}
\newcommand{\authorsize}{\fontsize{10pt}{12pt}\selectfont}
\newcommand{\absize}{\fontsize{11.5pt}{14pt}\selectfont}

\newbox\absbox
\def\abstract{\lrbox\absbox\minipage{\textwidth}%
  \normalfont%
  {\noindent\sffamily\bfseries\absize{ABSTRACT}}\par\vspace{10pt}\normalsize%
  }
\def\endabstract{\copyrightline\endminipage\endlrbox}

\def\keywords#1{%
  \gdef\@keywords{\small{\bfseries\sffamily KEYWORDS}\par\noindent\raggedright\noindent\sffamily{#1}}}
\let\@keywords\@empty

\skip\footins 22pt plus  8pt
%\gdef\footnoterule{}
\def\footnoterule{\kern-3\p@
  \hrule \@width 60pt \kern 2.6\p@}

\renewcommand{\thefootnote}{\fnsymbol{footnote}}
\long\def\@makefntext#1{\parindent 1em%
\noindent{$\m@th^{\@thefnmark}$}#1}

\def\corraddr#1{%
  \gdef\@corraddr{\small{\bfseries\sffamily {\corrauth}Correspondence}\par\noindent\raggedright\noindent\sffamily{#1}}%
    }
\let\@corraddr\@empty
\def\corrauth{\footnotemark[1]}

\def\address#1{%
  \gdef\@address{{\small\sffamily #1}}}
\let\@address\@empty

%\def\cgsn#1#2{%
%\gdef\@cgsn{%
%\small\noindent{\raggedright\bfseries\sffamily Contract/grant sponsor}\par\raggedright\noindent\sffamily{#1}\par\vspace{11pt}%
%\small\noindent{\raggedright\bfseries\sffamily Contract/grant number}\par\raggedright\noindent\sffamily{#2}\par\vspace{5pt}}}
%
%\def\cgs#1{%
%\gdef\@cgs{%
%\small\noindent{\raggedright\bfseries\sffamily Contract/grant sponsor}\par\raggedright\noindent\sffamily{#1}\par\vspace{5pt}}}
%
%\let\@cgsn\@empty
%\let\@cgs\@empty

\def\articletype#1{%
\gdef\@articletype{\authorsize\sffamily\noindent{#1}}}
\let\@articletype\@empty

\def\affilnum#1{${}^{#1}$}
\def\affil#1{${}^{#1}$}
\def\comma{${}^{\text{,}}$}

\renewcommand\maketitle{\par
  \begingroup
     \if@twocolumn
      \ifnum \col@number=\@ne
        \@maketitle
      \else
        \twocolumn[\@maketitle]%
       \fi
    \else
      \newpage
      \global\@topnum\z@   % Prevents figures from going at top of page.
      \@maketitle
    \fi
    \thispagestyle{title}\label{FirstPage}%\@corraddr\@cgs\@cgsn
  \endgroup
  %\setcounter{footnote}{0}%
  \global\let\address\relax
  \global\let\corraddr\relax
  \global\let\thanks\relax
  \global\let\maketitle\relax
  \global\let\articletype\relax
  \global\let\@maketitle\relax
  \global\let\@thanks\@empty
  \global\let\@author\@empty
  \global\let\@date\@empty
  \global\let\@title\@empty
  \global\let\@articletype\@empty
  \global\let\@address\@empty
  \global\let\@corraddr\@empty
  \global\let\title\relax
  \global\let\author\relax
  \global\let\date\relax
  \global\let\and\relax
}
\def\@maketitle{\vspace*{28pt}%
\null%
%\begin{center}
\@articletype\par
\vspace{9pt}
    {\raggedright\titlesize\sffamily\bfseries\noindent\@title \par}%
    \vskip 1.5em %
    \vskip -8pt
    {\large
      \lineskip .5em%
      \authorsize\sffamily\noindent\@author
      \par}%
      \vskip 7pt
{\small
      \lineskip .5em%
      %
        {\raggedright\sffamily\noindent\@address}
      \par}%
%\end{center}
    \vskip 34pt%
    {\noindent\usebox\absbox\par}
      {%
      \vspace{9pt}%
      {\noindent\@keywords}\par}
      {\vspace{5pt}%
      {\noindent\@corraddr}\par}
      \vspace{5pt}%
      %{\noindent\@cgs}}%
      %{\noindent\@cgsn}%
      %{\noindent\small\sffamily Received \dots}
      \vspace{22pt}
        \par%
  }

\def\startpage{\pageref{FirstPage}}
\def\endpage{\pageref{LastPage}}
\def\volumeyear{0000}
\def\volumenumber{00}

\gdef\copyrightline{Copyright \copyright\ \volumeyear\ John Wiley \& Sons, Ltd.}
\gdef\footercopyrightline{\copyright\ \volumeyear\ John Wiley \& Sons, Ltd.}
\def\runningheads#1#2{\markboth{{#1}}{{#2}}}

\def\ps@title{%
\def\@oddhead{%
\parbox[t]{\textwidth}{%
\mbox{}\hfill\begin{tabular}[t]{@{}r@{}}%
{\small\sffamily\journalname}\\[-1pt]
{\small\sffamily\emph{\journalabb} \volumeyear; \textbf{\volumenumber}:\startpage--\endpage}\\[-1pt]
{\small\sffamily DOI: 10.1002/\DOI}
\end{tabular}}}%
\let\@evenhead\@oddhead
\def\@oddfoot{\parbox[t]{\textwidth}{%
{\footnotesize\sffamily\copyrightline\hfill\numsize\textbf{\thepage}\\
\footnotesize\sffamily\textit{Prepared using \textsf{\journalclass} [Version: \update]\hfill}%
}}}
\let\@evenfoot\@oddfoot}

\def\ps@wpage{%
\let\@mkboth\@gobbletwo
\def\@evenhead{\small\sffamily{\rightmark}\hfill{\leftmark}}
\def\@oddhead{\small\sffamily{\leftmark}\hfill{\rightmark}}
\def\@evenfoot{\parbox[t]{\textwidth}{\sffamily\numsize\textbf{\thepage}\hfill%
\footnotesize \emph{\journalabb\ }\volumeyear; \textbf{\volumenumber}:\startpage--\endpage\ \footercopyrightline\\ %
\mbox{}\hfill DOI: 10.1002/\DOI\\
\mbox{}\hfill\footnotesize\textit{Prepared using \textsf{\journalclass}}}}
\def\@oddfoot{\parbox[t]{\textwidth}{\sffamily\footnotesize \emph{\journalabb\ }\volumeyear; \textbf{\volumenumber}:\startpage--\endpage\ \footercopyrightline%
\hfill\numsize\textbf{\thepage}\\%
\footnotesize DOI: 10.1002/\DOI\\
\textit{Prepared using \textsf{\journalclass}}}}%
}

\renewcommand{\@seccntformat}[1]{{\csname the#1\endcsname.}\hspace{0.5em}}

\newdimen\@bls
\@bls=\baselineskip

\renewcommand\section{\@startsection {section}{1}{\z@}%
                                   {2\@bls  plus .3\@bls minus .1\@bls}%
                                   {1\@bls\@afterindentfalse}%
                                   {\sffamily\bfseries\large\raggedright\protect\MakeTextUppercase}}
\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
                                     {\@bls plus .3\@bls minus .1\@bls}%
                                     {6pt\@afterindentfalse}%
                                     {\sffamily\bfseries\normalsize\raggedright}}
\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
                                     {\@bls plus .2\@bls}%
                                     {0.01pt}%
                                     {\sffamily\bfseries\normalsize\raggedright}}

\def\enumerate{\ifnum \@enumdepth >3 \@toodeep\else
      \advance\@enumdepth \@ne
      \edef\@enumctr{enum\romannumeral\the\@enumdepth}\list
      {\csname label\@enumctr\endcsname}{\usecounter
        {\@enumctr}\itemsep 0pt\parsep 0pt
         \def\makelabel##1{\hss\llap{##1}}}\fi}

\let\endenumerate =\endlist

\def\itemize{\ifnum \@itemdepth >3 \@toodeep\else \advance\@itemdepth \@ne
\edef\@itemitem{labelitem\romannumeral\the\@itemdepth}%
\list{\csname\@itemitem\endcsname}{\itemsep 0pt\parsep 0pt
\def\makelabel##1{\hss\llap{##1}}}\fi}

\let\enditemize =\endlist

\renewcommand{\thetable}{\Roman{table}}

\usepackage{caption}
\DeclareCaptionLabelSeparator{jwperiod}{.\hspace*{0.5ex}}
\captionsetup[figure]{font=small,labelfont={sf,bf},textfont=sf,labelsep=jwperiod,justification=centerlast,singlelinecheck=true}
\captionsetup[table]{font=small,labelfont={sf,bf},textfont=sf,labelsep=jwperiod,justification=centerlast,singlelinecheck=true}

\def\thmhead@plain#1#2#3{%
  \thmname{#1}\thmnumber{\@ifnotempty{#1}{ }{#2}}%
  \thmnote{ {\the\thm@notefont(#3)}}}

\newtheoremstyle{wiley}
{6pt plus 2pt minus 2pt}% space above
{6pt plus 2pt minus 2pt}% space below
{}% Body font
{}% Indent amount
{\itshape}% Theorem head font
{}% Punctuation after theorem head
{\newline}% Space after theorem head
{}% Theorem head spec

\renewenvironment{proof}[1][\proofname]{\par
  \pushQED{\qed}%
  \normalfont \topsep6\p@\@plus6\p@\relax
  \trivlist
  \item[\hskip\labelsep
        \itshape
    #1\@addpunct{}]\mbox{}\newline\ignorespaces
}{%
  \popQED\endtrivlist\@endpefalse
}

\theoremstyle{wiley}

\def\ack{\section*{ACKNOWLEDGEMENT}}
\def\acks{\section*{ACKNOWLEDGEMENTS}}

\renewcommand\refname{REFERENCES}

\renewenvironment{thebibliography}[1]{%
\section*{\refname}
\list{{\arabic{enumi}}}{\def\makelabel##1{\hss{##1.}}\topsep=0\p@\parsep=0\p@
\partopsep=0\p@\itemsep=0\p@
\labelsep=1ex\itemindent=0\p@
\settowidth\labelwidth{\normalsize[#1]}%
\leftmargin\labelwidth
\advance\leftmargin\labelsep
\advance\leftmargin -\itemindent
\usecounter{enumi}}\normalsize
\def\newblock{\ }
\sloppy\clubpenalty4000\widowpenalty4000
\sfcode`\.=1000\relax}{\endlist}

\def\biog{\section*{Author's Biography}}
\def\biogs{\section*{Authors' Biographies}}

\AtEndDocument{%
\label{LastPage}}

\hyphenation{Tele-com-mu-ni-ca-tions}
\hyphenation{com-mu-ni-ca-tions}

\pagestyle{wpage}
\twocolumn
\normalsize
\sloppy
